6G Integrated Sensing and Communication: From Vision to Realization

Integrated sensing and communications (ISAC) will be deployed into cellular communication systems possibly already with 5G-A and surely in 6G. This paper discusses ISAC use cases, key technology building blocks for system design with solutions and open research questions. Furthermore, we introduce our proof-of-concept (PoC) based on commercially available 5G communications hardware at mm-Wave frequencies, with sensing-specific algorithmic extensions. This new ISAC PoC can perform jointly high data-rate communications and OFDM radar sensing in the same frequency band. Initial pedestrian detection results are shown, indicating the practicability of ISAC in future cellular networks. The results also indicate our achievable sensing range and provide hints to the achievable range estimation accuracy, based on the stability of the PoC system communications hardware.

==> 6G Integrated Communication and Sensing From Vision to Realization/Content/Abstract.tex <==
\begin{abstract}
Integrated sensing and communications (ISAC) will be deployed into cellular communication systems possibly already with 5G-A and surely in 6G.
This paper discusses ISAC use cases, key technology building blocks for system design with solutions and open research questions. Furthermore, we introduce our \gls{poc} based on commercially available 5G communications hardware at mm-Wave frequencies, with sensing-specific algorithmic extensions. This new ISAC \gls{poc} can perform jointly high data-rate communications and OFDM radar sensing in the same frequency band. Initial pedestrian detection results are shown, indicating the practicability of ISAC in future cellular networks. The results also indicate our achievable sensing range and provide hints to the achievable range estimation accuracy, based on the stability of the \gls{poc} system communications hardware.
\end{abstract}
%\vspace{-0.78mm}

==> 6G Integrated Communication and Sensing From Vision to Realization/Content/Acknowledgment.tex <==
\section*{Acknowledgments}
This work was developed within the KOMSENS-6G project, partly funded by the German Ministry of Education and Research under grant 16KISK112K.

%\balance

==> 6G Integrated Communication and Sensing From Vision to Realization/Content/Acronyms.tex <==
\newacronym{agv}{AGV}{automated guided vehicle}
\newacronym{bf}{BF}{beamforming}
\newacronym{bs}{BS}{base station}
\newacronym{dft}{DFT}{Discrete Fourier Transform}
\newacronym{dl}{DL}{downlink}
\newacronym{e2e}{E2E}{end-to-end}
\newacronym{fmcw}{FMCW}{frequency modulated continuous wave}
\newacronym{isac}{ISAC}{Integrated Sensing and Communication}
\newacronym{kf}{KF}{Kalman Filter}
\newacronym{ofdm}{OFDM}{orthogonal frequency-division multiplexing}
\newacronym{papr}{PAPR}{peak-to-average power ratio}
\newacronym{poc}{PoC}{proof-of-concept}
\newacronym{qos}{QoS}{quality of service}
\newacronym{scfde}{SC-FDE}{single carrier frequency domain equalization}
\newacronym{uav}{UAV}{unmanned aerial vehicle}
\newacronym{ue}{UE}{user equipment}
\newacronym{ul}{UL}{uplink}
\newacronym{semf}{SeMF}{sensing management function}
\newacronym{snr}{SNR}{signal-to-noise ratio}
\newacronym{tdd}{TDD}{time division duplex}
\newacronym{tx}{TX}{transmit}





==> 6G Integrated Communication and Sensing From Vision to Realization/Content/Building_Blocks.tex <==
\section{Technology Building Blocks}%, Research Challenges, and Solutions}
\label{sec:building_blocks}

%\begin{figure*}
%    \begin{center}
%        \includegraphics[width=0.75\textwidth]{figures/Sesning_variants_overview.png}
%    \end{center}
%\caption{[Placeholder] –Overview on different sensing variants.}
%  \label{fig:variants_overview}
%\end{figure*}

Sensing in cellular systems can be achieved by different architectures. %, as illustrated by Fig.~\ref{fig:variants_overview}. 
If the sensing processing resides in the \gls{bs}, the system has lighter signaling overhead and less demands concerning \gls{ue} complexity and battery consumption. Sensing transmitters located at the \gls{bs} offer a larger range  (due to higher transmit powers and advantageous placement). 
%\todo[inline]{SM: in my opinion, Figure 1 should not be added in such a short paper (because it would require a longer description of at least all the options). I would have a smaller figure with the mono-static network-based architecture, that is the only one we really consider here, or simply use current Figure 2.}
%
Mono-static sensing requires an almost full duplex capability, where the self-interference can be reduced by a slightly separated receive array in combination with regular communications \gls{tdd} operation, as we will discuss in~\ref{sec:Poc_Realization}. 
Moreover, mono-static solutions offer easier use of data-aided sensing, which has the opportunity to avoid sensing overhead in case an active communication transmission is ongoing in the sensing direction of interest.
Bi-static sensing can avoid this issue, but requires receiving sensing entities to mute transmissions, which reduces the temporal availability of the \gls{isac} system, and thus increases the additional overhead for sensing on top of the communication system. 
Using both \gls{ue}s and \gls{bs} is a further bi-static sensing alternative which requires the availability of a \gls{ue} at the location of interest.
%\todo[inline]{SM: removed the sentence about UE-based sensing, but feel free to restore it.}

In our \gls{poc} we focus on the network-based mono-static \gls{isac}. %This variant has a low introduction hurdle in 5G-Advanced systems with low standardization impact as dedicated sensing signals can be inserted as dummy data by the \gls{bs} scheduler \egc within single \gls{ofdm} symbols, so-called mini-slots.
%\todo[inline]{SM: do we want to mention the ``low standardization impacts''? It could be a rabbit hole though, thus I would prefer to omit the standard-related part in this paper and remove its mention.}
Fig.~\ref{fig:sys_overview} displays a simplified \gls{e2e} system overview (and further more our used \gls{poc} interfaces and building blocks as described in ~\ref{sec:Poc_Realization} are marked) with the \gls{bs} split architecture with radio unit (RU), distributed unit (DU) and central unit (CU). It remains a research and standardization challenge to come up with accepted \gls{isac} channel models which serve well for simulating both communication and sensing performance offering some level of statistical abstraction. 
%The MaxRay multi-modal ray-tracing tool \cite{arnold2022maxray} offers to jointly simulate RF propagation and other modalities: vision and lidar. This is useful for cross-modal learning \cite{alloulah2022}, which helps to make labeling for AI/ML-based detection techniques scalable.
Agreed communication channel models for performance benchmarks are statistically based; they so far fail to support the required sensing features of full geometrical consistency in combination with a radar cross section parameter. A statistical model for \gls{isac} fixing those issues with the option of ray-tracing-assisted cluster placement could be an attractive way forward for 3GPP and thus needs to be studied in Rel. 19, where Ch.~8 in~\cite{3gppchan} could serve as a starting point.
%\todo[inline]{SM: given the 4 page limit, I am not sure if the last reference to \cite{arnold2022maxray,alloulah2022} are really necessary. We can however point to 38.901 that is already addressing this in the current Ch. 8. I can rephrase this part, if you are ok with it. 
%\\TW: If we also drop these 2 references the theme around ``solutions and research challenges`` becomes very thin and so I'd like to keep it. I have also added your proposed reference. Feel free to modify that part, e.g. the sentence above the commenting box.
%\\SM: as you prefer, to me it's still a bit stretched, but as you prefer!}

To implement \gls{isac}, radio front-end design must take into account new challenges and review solutions for ones already well investigated.
Full duplex requires to deal with self-interference. We circumvent this issue by using a separated \emph{Sniffer} RU for reception of the reflections. With appropriate array design and self-interference compensation mechanisms the communication array and the Sniffer may be integrated as subpanels into a single RU (or alternatively, based on the split processing interfaces described in \ref{sec:Poc_Realization} be placed further apart for bi-/multi-static operation). Note that during \gls{ul}, both arrays could be used to improve diversity and \gls{snr} for the communication mode. Another issue arises from the presence of analog and hybrid \gls{bf} in FR2 and even Golden Band frequencies. To get a radar image of the environment with pre-defined grid of beams codebooks implemented in wireless products, the angular domain must be properly sampled and interpolated. SARA \cite{sara2022} addresses this and defines how lossless reconstruction of the array's angular response can be achieved by uniform sampling in the \gls{dft} beamspace of the system's sum co-array and its corresponding interpolation.

%Another front-end issue is the likely presence of hybrid \gls{bf} in FR2 and even Golden Band frequencies. This poses a spatial sampling problem, which can be elegantly addressed by the SARA technique \cite{sara2022}, which uses a \gls{bf} codebook with uniform spacing in normalized angular frequency, instead of uniform angle and reconstructs by interpolation with Dirichlet kernels.

Scheduling of both communication as well as sensing signals in the same carrier poses new design questions and opportunities. The proportional fair metric in communication schedulers \cite{pf2014} should be expanded towards integrating (i)~legacy communications and (ii)~to-be-defined sensing \gls{qos}. The \gls{e2e} network architecture of 5G systems needs to be expanded by new network functionalities dedicated to sensing, which we could denote \gls{semf}. This central function will be responsible for aggregating sensing information from \glspl{bs} and \gls{ue}s, and providing high-level resource allocation management to cells involved in sensing operations based on sensing \gls{qos}.
%\todo[inline]{SM: this last following paragraph may be problematic given current IPR brainstorming. I would omit it}
%Furthermore, service exposure has to be provided in the \gls{e2e} architecture to allow sensing applications to access the information obtained by the network with appropriate controlled level of privacy.

With 6G as AI-native air interface, AI/ML for sensing can leverage available AI-hardware acceleration and is attractive to be used for tasks such as object detection and classification, both locally in the \gls{bs} or centrally in the \gls{semf}.

==> 6G Integrated Communication and Sensing From Vision to Realization/Content/Conclusion.tex <==
\section{Conclusion}\label{sec:Conclusion}

The background for system design for \gls{isac} in cellular 5G-A and 6G systems has been discussed. 
%, first with a brief overview on different possible sensing variants with \gls{ue} and \gls{bs}. 
Technical building blocks with solution options and research challenges have been addressed. %(removed by MH) \gls{isac} poses a big opportunity to expand cellular system service capabilities and to offer large scale services, leveraging the cellular economy of scale. 
Then, a novel \gls{poc} implementation with results has been presented, which shows that existing millimeter-wave 5G hardware can provide a good basis for adding sensing capabilities on top and that pedestrians can be detected well and become separated from clutter with appropriate algorithms.


==> 6G Integrated Communication and Sensing From Vision to Realization/Content/Introduction.tex <==
\section{Introduction}\label{sec:intro}
6G cellular communication is predicted to be commercially ready in 2030. A key element of its vision is forming around the connection of different worlds \cite{viswanathan2020}. This is a representation of the physical/biological world in software,  thus digital twinning. Digital twins can play an important role especially in the industrial sector to enhance productivity, safety and security. In each wireless generation, larger bandwidths have been used, denser networks, more processing capabilities and a larger number of antennas. Under these trends with ubiquitously deployed cellular communication systems in place, the integration of RF sensing is becoming more and more attractive to extend the network service capabilities and to enable the digital twins with the necessary context information from the environment. The 6G network will become the sensor \cite{de2021convergent, wei2022toward, wild2021joint}, building on cellular system strengths such as interference management, wide area coverage and tightly controlled and scheduled operation. 5G systems already have active localization capabilities \cite{henninger2022probabilistic}, where positioning reference signals are transmitted from \glspl{ue} or \glspl{bs}, also denoted as gNBs. Furthermore, for 5G systems, 3GPP standardization has identified possible use cases for \gls{isac} \cite{3gpp}, which would allow to detect also objects which are not connected to the network. There are large public funded projects, e.g. \cite{hexa_x}, which address the collaborative work towards \gls{isac} technologies and system design for the coming years.

In this paper we discuss 6G \gls{isac} starting from spectrum and key use cases. Technology building blocks, available solutions and research challenges are addressed and finally we describe a novel real-time \gls{isac} \gls{poc}, which builds upon commercially available 5G communications hardware in combination with dedicated sensing processing elements. We make use of the communications split processing architecture interfaces for sensing purposes and \gls{ofdm} radar processing algorithms \cite{Braun2014_OFDM_Radar}, enhanced by clutter removal and tracking algorithms. In our \gls{poc}, sensing can be carried out with down to 0\% sensing overhead on top of running communication services. We show example results for human detection hinting to achievable range and range estimation stability and accuracy.

==> 6G Integrated Communication and Sensing From Vision to Realization/Content/Overview.tex <==
\section{Basic Overview overview on 6G ISAC}\label{sec:overview}
\begin{figure*}[!t]
    \begin{center}
        \includegraphics[width=0.95\textwidth]{figures/SysOverview_v03.png}
    \end{center}
\caption{System overview incl. our \gls{poc} processing blocks and associated research challenges (red) – mono-static example.}
  \label{fig:sys_overview}
\vspace{-5mm}
\end{figure*}
\gls{isac} makes very efficient use of spectrum as, due to its integrated nature, the same bands with the same carriers can be used for both communication and sensing purposes, and the multiplexing capabilities of cellular systems (\egc due to \gls{ofdm} waveforms) can efficiently trade-off service qualities both for communications as well as the new to-be-introduced sensing service qualities. The spectrum choice dominates the system capabilities. 5G capacity layers are in the so-called FR1 (frequency range 1) bands below 5 GHz and use bandwidths up to 100 MHz. FR2 in the millimeter frequency ranges starting at around 24 GHz offer bandwidths up to 800 MHz and are more attractive for sensing due to the higher range resolution. For 6G, the main capacity layer, the ``Golden Band", is expected to be in 6-14 GHz and may offer up to 400 MHz of bandwidth, making it attractive for wide-area sensing. In order to re-use 5G site-grids, we can expect massive MIMO \glspl{bs} with around 1024 antenna elements (offsetting coverage drawbacks relative to FR1), thus we can also leverage large antenna apertures for angular resolution. Refarming and spectrum sharing of lower FR1 bands may also happen but will come with limited available bandwidths. This means that we can see the Golden Band and FR2 millimeter wave spectrum as the strongest sensing introduction candidates in 6G. Sub-THz technologies with carrier frequencies \textgreater100 GHz are also highly discussed for 6G and would offer huge bandwidths. Looking at the commercial introduction of 5G, the FR1 band was dominating over the FR2 band due to better coverage. If 6G deployments will be driven along the commercial needs of communication systems first, we can assume that also sub-THz sensing may initially not play the strongest role in early 6G.

We can expect that the key \gls{isac} use cases will be driven and stimulated by the frequency-dependent deployment scenarios. Micro-cellular deployments mainly rely on FR2 (and alternatively/later sub-THz) and will be used indoor and in hot-spot areas. In factory floor environments, pedestrians, passive factory objects or other moving objects (such as robots, \glspl{agv} and fork lifts) can be detected . This could enhance safety in industrial environments. Macro-cellular deployments will dominate outdoors, where mainly the Golden Bands are of key interest for sensing. Traffic monitoring, highway intrusion detection, roadside safety, drone/\gls{uav} intrusion detection or tracking are all examples of possible use cases. Cellular networks can provide the infrastructure-based sensing where local sensors would be limited by not being able to ``look around the corner" from the device point of view.

Regarding waveforms for \gls{isac}, the aforementioned \gls{ofdm} is fully established in 4G and 5G communication systems and is also gaining more momentum in the radar world. Therefore, \gls{ofdm} is an attractive option to multiplex communication and sensing services in the same carrier band. Its only drawback is the \gls{papr}, so in case of \egc higher carrier frequencies, communication systems may use \gls{scfde} as an alternative, which could leverage the same frequency domain sensing processing as \gls{ofdm}. Other waveform alternatives (such as time-multiplexing of communication waveforms with \gls{fmcw}) are of course not ruled out and can also be studied.

==> 6G Integrated Communication and Sensing From Vision to Realization/Content/PoC_Realization.tex <==
\section{Proof of Concept Architecture}\label{sec:Poc_Realization}
%\begin{figure}
%    \begin{center}
%      \includegraphics[width=1.0\linewidth]{figures/Architecture_block_diagram.png}
%    \end{center}
%    \caption{Architecture of the \gls{poc}. Top part shows communication system, extensions that enable ISAC capability below.\todo[inline]{redo figure properly in inkscape}}
%    \label{fig:arch}
%    \vspace{-4mm}
%\end{figure}
A major design goal of the \gls{isac} architecture is to re-use as much of the communication hardware as possible for sensing purposes.
The \gls{ofdm} radar approach~\cite{Braun2014_OFDM_Radar} uses the frequency domain \gls{tx} reference signal and frequency domain reflected signal as inputs into the radar processing chain.
Looking at possible functional splits for 5G~\cite{Larsen_2019_Functional_Splits}, using Option 7-2 (FFT/iFFT done in RU, frequency-domain IQ transported on fronthaul) allows use of the same type of RU for both communication and sensing, and using the fronthaul between DU and RU as the input to \gls{ofdm} radar processing.

\Cref{fig:sys_overview} shows also the architecture of our \gls{poc}.
The building blocks in green are based on a commercial 5G FR2 communication system we use as a foundation.
To enable \gls{isac} we extend this system with (i) a dedicated RU called \emph{Sniffer} of the same type as the communication RU and (ii) a server called Sensing Processing Unit (\emph{SPU}) running our real-time \gls{ofdm} radar processing software, highlighted in orange.
%\todo[inline]{TW: Some redundancy with the sniffer-array part in section III}
While the gNB RU is operating in TDD mode (4:1 DL/UL ratio), the Sniffer is always in \gls{ul}-mode, thus it receives both reflected signals and uplink signals from \glspl{ue}.

The communication setup uses eCPRI~\cite{eCPRI_2_0_Spec} over optical fiber (25 GE) to carry Sync-, Management-, Control- and User-planes.
A fiber-optical splitter on the DU$\rightarrow$RU fiber allows us access to the \gls{tx} waveform and \gls{bf} information used by the communication setup.
The Sniffer is directly controlled by the SPU, which switches beams and requests the radio resources to be received over Control-plane, and receives IQ-data of the reflected signal via User-plane. 
%
Both RUs are connected via fiber to a common sync source (5G system module), synchronizing both RUs via PTP~\cite{PTPv2_spec} and SyncE~\cite{SyncE_spec}, resulting in a synchronization jitter of $\approx$40ps between gNB RU and Sniffer.
%\todo[inline]{TW: PTP and SyncE are not spelled out, as well as CUDA, GPU and SFP below and eCPRI above... Maybe some of the abbreviations can be assumed to be commonly known? But probably not all of them...}
The SPU server hardware uses 25 GE network cards to allow fronthaul access of gNB RU and Sniffer and synchronization of the SPU to the same PTP source (5G system module) as the RUs.
A CUDA capable GPU is used for \gls{ofdm} radar processing and visualization.% of the sensing results. 
%
%
\begin{figure*}
  \begin{subfigure}[t]{0.22\linewidth}
    \begin{center}
      \includegraphics[width=1.0\linewidth,clip,trim={0mm 20mm 30mm 20mm}]{figures/lab-walking-photo-1.jpg}
    \end{center}
    \caption{Photo from the RUs (gNB RU top left, Sniffer top right) in the direction of the beam.}
    \label{fig:res_lab_walking_photo}
  \end{subfigure}\enspace%
  \begin{subfigure}[t]{0.35\linewidth}
    \begin{center}
      \includegraphics[width=1.0\linewidth]{figures/lab-walking-SPU-core-screenshot.png}
    \end{center}
    \caption{Realtime visualization by our SPU software after \emph{Peak Extraction and Interpolation}. The target corresponding to the human \textbf{H} is highlighted.}
    \label{fig:res_lab_walking_spu_core}
  \end{subfigure}\enspace%
  \begin{subfigure}[t]{0.43\linewidth}
    \begin{center}
      \includegraphics[width=1.0\linewidth,clip,trim={0mm 10mm 0mm 0mm}]{figures/lab-walking-HOS-screenshot.png}
    \end{center}
    \caption{Range and speed of the human over the past 10 seconds after \emph{Target Tracking}.}
    \label{fig:res_lab_walking_hos}
  \end{subfigure}
  \caption{Testing our ICAS PoC using a ``Walking Human'' scenario, with person \textbf{H} walking towards and away from the RUs. Clutter removal (main clutter \textbf{C} highlighted) was active.}
  \label{fig:res_lab_walking_scenario}
  \vspace{-5mm}
\end{figure*}
%

The SPU processing chain comprises the following steps:
\begin{compactitem}
\item \emph{Reference and Reflected Signal Reception}. Receive and preprocess eCPRI packets from gNB RU and Sniffer.
Each radio frame is an $N\times M$ matrix, where $N$ is the number of subcarriers (SC) in each symbol, and $M$ is the number of symbols in the radio frame.
\item \emph{Channel Computation}. Perform resource-element-wise division of the reflected signal by the reference signal.
\item \emph{Clutter Removal}. To isolate targets, it is crucial to remove signal contributions resulting from reflections from objects not of interest for the sensing task.
We record the channel of the reference scenario during system calibration and subtract it from the reflected signal at runtime.
\item \emph{Range/Doppler Periodogram Computation}. Perform $N$ FFTs on the channel, followed by $M$ iFFTs on the result.
The squared magnitude of each element of the result of the FFTs and iFFTs operations are computed, resulting in a 2D-periodogram, containing Doppler and range information for the processed radio frame.
\item \emph{Peak Extraction and Interpolation}. Elements in the periodogram that exceed a configurable threshold are potential targets.
The remaining elements usually form clusters in the range and Doppler domain, caused by the same object.
We extract the local maxima of these clusters and use them to construct the target list (sorted by element value, which corresponds to received power).
\item \emph{Target Tracking}. Detected targets are optionally tracked by means of a simple \gls{kf}.% using a constant velocity motion model. %~\cite{welch1995introduction}.  
\end{compactitem}

\section{First Results}
\label{sec:Results}

Using the system described in the previous section in a lab, we track a walking human.
The system operates at a center frequency of 27.6 GHz with 200 MHz bandwidth and a $\mu=3$ numerology (120 kHz SC spacing, 1120 symbols per frame).
In this experiment we use a test signal sent by the gNB RU (instead of a UE connection), which uses all SCs within the DL part of the radio frame modulated with 16-QAM.
The beam ($14^\circ$ of half-power horizontal beam width) is kept static during the test.
Both RUs are mounted at a height of ca. 1.9m, with a distance of $\approx$40cm between gNB RU and Sniffer.

\Cref{fig:res_lab_walking_scenario} shows (a) a photo of the scenario, (b) the SPU real-time visualization ``radar view'', with the person corresponding to the green arc within the beam cone, and (c) the distance from the RU and speed over the past 10 seconds of the strongest reflector (the person in this experiment), filtered by the  \gls{kf}.

\Cref{fig:res_pgram_clutter} shows the effect of clutter removal -- indoor environments often contain objects (such as a metal cabinet and support pillar \textbf{C}) that cause stronger reflections than a human.
With clutter removal, the effects of these reflectors are removed, resulting in a periodogram with only the target \textbf{H} clearly visible.
This makes algorithms which use the results of OFDM radar as inputs (\egc Target Tracking) more robust.

%Finally, two numerical examples for the achievable range accuracy of our \gls{poc} are given. Computing the standard deviation of the range estimation for sensing a static human \textbf{H} at a distance of 3m from the sniffer amounts to $\sigma_{H} = 5$mm, while sensing the strong clutter \textbf{C} ca. 5.5m away from the sniffer yields $\sigma_{C} = 2$mm (both values without tracking). Those results give an indication about the accuracy and stability of our system.
In our first setup evaluations, we experienced a range standard deviation of $\sigma_{H} = 5$ mm for a human target at $r_H^0 = 3$ m range, while a strong clutter component at ca. 5.5~m range yields $\sigma_{C} = 1$ mm, before any tracking algorithms are considered. Given the estimated \gls{snr} $\gamma_H(r_H^0) = 10^{6.885}$ at $r_H^0$ range for humans, and assuming free space path loss exponent $\eta = 2$, a rough assumption of the \gls{snr} experienced at a generic range $r$ for human sensing with our setup can be written as
\begin{equation}
\gamma_H(r) = \gamma_H(r_H^0) \cdot (r_H^0/r)^{2 \eta} \;.
\end{equation}
Assuming a minimum \gls{snr} (after combining gains) $\gamma_0 = 10^{1.7}$ in order to obtain a reasonable spectral estimation performance~\cite{MUSIC_collapse}, one can determine the achievable range by our setup on human sensing as
\begin{equation}
r_H^* = \sqrt[2\eta]{\frac{\gamma_H(r_H^0)}{\gamma_0}} \cdot r_H^0 \approx 60\; m \; .
\end{equation}

\begin{figure}
    \begin{center}
      \includegraphics[width=1.0\linewidth,clip,trim={3mm 3mm 5mm 4mm}]{figures/lab-walking-clutter.pdf}
    \end{center}
    \caption{Periodograms of same radio frame with and without clutter removal. Clutter \textbf{C} produces much stronger reflection than human \textbf{H}.}
    \label{fig:res_pgram_clutter}
  \vspace{-5mm}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main_jcas_poc"
%%% End:


==> 6G Integrated Communication and Sensing From Vision to Realization/EuMW_modify_IEEEtran_18b_CTAN_V4.tex <==
% EuMW_modify_IEEEtran_18b_CTAN_V4.tex
%         created by Causal Productions Pty Ltd, 
%	  http://www.causalproductions.com
%	  info@causalproductions.com
%
%	  This file is Copyright 2017-2018 Causal Productions Pty Ltd.
%	  Permission is granted to use this file and its associated files
%	  for conferences for which Causal Productions has been contracted
%	  to prepare the conference proceedings.
%
% This file contains format modifications to the standard IEEE style file
% called IEEEtran.cls version 1.8b, as hosted on CTAN at the following URL:
%	http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/
%
% The purpose of the format modifications is to implement a paper format
% traditionally used by EuMW conferences, which differs from the standard
% IEEE conference paper format in various ways, such as font sizes.
%  
% This file is NOT intended to be used with the different IEEEtran.cls version 1.8
% that is distributed by IEEE at the following URL:
%	http://www.ieee.org/web/publications/pubservices/confpub/AuthorTools/conferenceTemplates.html
% Despite having the same version number 1.8, the CTAN and IEEE versions are
% different and this particular modification file is designed only for the 
% CTAN version.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter

% EuMW: override title block font sizes
% formats the Title, authors names, affiliations and special paper notice
% THIS IS A CONTROLLED SPACING COMMAND! Do not allow blank lines or unintentional
% spaces to enter the definition - use % at the end of each line
\def\@maketitle{\newpage
\bgroup\par\addvspace{0.5\baselineskip}\centering%
\ifCLASSOPTIONtechnote% technotes
   {\bfseries\large\@IEEEcompsoconly{\sffamily}\@title\par}\vskip 1.3em{\lineskip .5em\@IEEEcompsoconly{\sffamily}\@author
   \@IEEEspecialpapernotice\par{\@IEEEcompsoconly{\vskip 1.5em\relax
   \@IEEEtitleabstractindextextbox{\@IEEEtitleabstractindextext}\par
   \hfill\@IEEEcompsocdiamondline\hfill\hbox{}\par}}}\relax
\else% not a technote
   \vskip0.2em{\EuMWtitlesize\ifCLASSOPTIONtransmag\bfseries\LARGE\fi\@IEEEcompsoconly{\sffamily}\@IEEEcompsocconfonly{\normalfont\normalsize\vskip 2\@IEEEnormalsizeunitybaselineskip
   \bfseries\Large}\@title\par}\vskip1.0em\par% CAUSAL PRODUCTIONS change on this line
   % V1.6 handle \author differently if in conference mode
   \ifCLASSOPTIONconference%
      {\@IEEEspecialpapernotice\mbox{}\vskip\@IEEEauthorblockconfadjspace%
       \mbox{}\hfill\begin{@IEEEauthorhalign}\@author\end{@IEEEauthorhalign}\hfill\mbox{}\par}\relax
   \else% peerreviewca, peerreview or journal
      \ifCLASSOPTIONpeerreviewca
         % peerreviewca handles author names just like conference mode
         {\@IEEEcompsoconly{\sffamily}\@IEEEspecialpapernotice\mbox{}\vskip\@IEEEauthorblockconfadjspace%
          \mbox{}\hfill\begin{@IEEEauthorhalign}\@author\end{@IEEEauthorhalign}\hfill\mbox{}\par
          {\@IEEEcompsoconly{\vskip 1.5em\relax
           \@IEEEtitleabstractindextextbox{\@IEEEtitleabstractindextext}\par\hfill
           \@IEEEcompsocdiamondline\hfill\hbox{}\par}}}\relax
      \else% journal, peerreview or transmag
         \ifCLASSOPTIONtransmag
            % transmag also handles author names just like conference mode
            % it also uses \@IEEEtitleabstractindextex, but with one line less
            % space above, and one more below
           {\@IEEEspecialpapernotice\mbox{}\vskip\@IEEEauthorblockconfadjspace%
            \mbox{}\hfill\begin{@IEEEauthorhalign}\@author\end{@IEEEauthorhalign}\hfill\mbox{}\par
           {\vspace{0.5\baselineskip}\relax\@IEEEtitleabstractindextextbox{\@IEEEtitleabstractindextext}\vspace{-1\baselineskip}\par}}\relax
         \else% journal or peerreview
           {\lineskip.5em\@IEEEcompsoconly{\sffamily}\sublargesize\@author\@IEEEspecialpapernotice\par
           {\@IEEEcompsoconly{\vskip 1.5em\relax
            \@IEEEtitleabstractindextextbox{\@IEEEtitleabstractindextext}\par\hfill
            \@IEEEcompsocdiamondline\hfill\hbox{}\par}}}\relax
         \fi
      \fi
   \fi
\fi\par\addvspace{0.0\baselineskip}\egroup}% CAUSAL PRODUCTIONS change on this line, reduce the vspace from 0.5\baselineskip to 0.0

% EuMW: change font sizes in the document
%	paper title is 24pt
%	bib items are 9pt 
%	author names are 11pt
%	author affils are 10pt
%	captions of figs and tables are 9pt
\def\EuMWtitlesize{\@setfontsize{\EuMWtitlesize}{24}{24pt}}% CAUSAL PRODUCTIONS change on this line
\def\EuMWauthorsize{\@setfontsize{\EuMWauthorsize}{11}{11pt}}% CAUSAL PRODUCTIONS change on this line
\def\EuMWaffilsize{\@setfontsize{\EuMWaffilsize}{10}{10pt}}% CAUSAL PRODUCTIONS change on this line
\def\EuMWcaptionsize{\@setfontsize{\EuMWcaptionsize}{9}{10pt}}% CAUSAL PRODUCTIONS change on this line
\def\EuMWbibsize{\@setfontsize{\EuMWbibsize}{8}{10pt}}% CAUSAL PRODUCTIONS change on this line

\def\@IEEEauthorblockNstyle{\EuMWauthorsize\@IEEEcompsocnotconfonly{\sffamily}\@IEEEcompsocconfonly{\large}}%CAUSAL PRODUCTIONS removed sublargesize to get correct EuMWauthorsize
\def\@IEEEauthorblockAstyle{\EuMWaffilsize\@IEEEcompsocnotconfonly{\sffamily}\@IEEEcompsocconfonly{\itshape}\@IEEEcompsocconfonly{\large}}%CAUSAL PRODUCTIONS removed normalsize to get correct EuMWaffilsize
% The default if the user does not use an author block
\def\@IEEEauthordefaulttextstyle{\EuMWauthorsize\@IEEEcompsocnotconfonly{\sffamily}\sublargesize}%CAUSAL PRODUCTIONS

\def\thebibliography#1{\section*{\refname}%
    \addcontentsline{toc}{section}{\refname}%
    % V1.6 add some rubber space here and provide a command trigger
    \EuMWbibsize\@IEEEcompsocconfonly{\small}\vskip 0.3\baselineskip plus 0.1\baselineskip minus 0.1\baselineskip% CAUSAL PRODUCTIONS change on this line
    \list{\@biblabel{\@arabic\c@enumiv}}%
    {\settowidth\labelwidth{\@biblabel{#1}}%
    \leftmargin\labelwidth
    \advance\leftmargin\labelsep\relax
    \itemsep \IEEEbibitemsep\relax
    \usecounter{enumiv}%
    \let\p@enumiv\@empty
    \renewcommand\theenumiv{\@arabic\c@enumiv}}%
    \let\@IEEElatexbibitem\bibitem%
    \def\bibitem{\@IEEEbibitemprefix\@IEEElatexbibitem}%
\def\newblock{\hskip .11em plus .33em minus .07em}%
% originally:
%   \sloppy\clubpenalty4000\widowpenalty4000%
% by adding the \interlinepenalty here, we make it more
% difficult, but not impossible, for LaTeX to break within a reference.
% IEEE almost never breaks a reference (but they do it more often with
% technotes). You may get an underfull vbox warning around the bibliography, 
% but the final result will be much more like what IEEE will publish. 
% MDS 11/2000
\ifCLASSOPTIONtechnote\sloppy\clubpenalty4000\widowpenalty4000\interlinepenalty100%
\else\sloppy\clubpenalty4000\widowpenalty4000\interlinepenalty500\fi%
    \sfcode`\.=1000\relax}

% EuMW: make a version of \@makecaption which uses \EuMWcaptionsize
%	and which formats all figure captions as justified if long, centered if short,
%	and formats all table captions using identical format to figure captions.
%	We are discarding the archaic small-caps format of table captions which was so hard to read.
%
\long\def\@makecaption#1#2{%
% test if is a for a figure or table
%  if figure, must make a vertical space before caption to separate caption from figure content
%  if table, must make a vertical space after caption to separate caption from table content
\ifx\@captype\@IEEEtablestring%
\par\@IEEEtabletopskipstrut% strut used to align table caption with facing column
\else
\@IEEEfigurecaptionsepspace
\fi
% 3/2001 use footnotesize, not small; use two nonbreaking spaces, not one
\setbox\@tempboxa\hbox{\normalfont\footnotesize {#1.}\nobreakspace\nobreakspace #2}%
\ifdim \wd\@tempboxa >\hsize%
% if caption is longer than a line, let it wrap around
\setbox\@tempboxa\hbox{\normalfont\footnotesize {#1.}\nobreakspace\nobreakspace}%
\parbox[t]{\hsize}{\normalfont\footnotesize\noindent\unhbox\@tempboxa#2}%
% if caption is shorter than a line, center if conference, left justify otherwise
\else
\ifCLASSOPTIONconference \hbox to\hsize{\normalfont\footnotesize\hfil\box\@tempboxa\hfil}%
\else \hbox to\hsize{\normalfont\footnotesize\box\@tempboxa\hfil}%
\fi\fi
% test if is a for a figure or table
%  if figure, must make a vertical space before caption to separate caption from figure content
%  if table, must make a vertical space after caption to separate caption from table content
\ifx\@captype\@IEEEtablestring%
\@IEEEtablecaptionsepspace
\else
\fi}

% EuMW: define table-caption-to-table separation separately from figure-to-figure-caption separation
\newlength\tablecaptiontotableskip
\newlength\figuretocaptionskip
% but only \abovecaptionskip is used above figure captions and *below* table
% captions
\setlength\tablecaptiontotableskip{0.5\baselineskip}% 0.5bs gives about 3mm from caption baseline to table
\setlength\figuretocaptionskip{0.0\baselineskip}% 0bs gives about 3mm from figure to caption top of lc letters, which matches appearance of table.
\def\@IEEEfigurecaptionsepspace{\vskip\figuretocaptionskip\relax}%
\def\@IEEEtablecaptionsepspace{\vskip\tablecaptiontotableskip\relax}%

% EuMW: Use Michael Shells suggested fix to reduce the space around emdash following Abstract and Index Terms headings
\def\abstract{\normalfont%
\@IEEEabskeysecsize\bfseries\textit{\abstractname}\,\bfseries\textit{---}\,%
\@IEEEgobbleleadPARNLSP}%
\def\endabstract{\relax\vspace{0ex}\par%
\normalfont\normalsize}%

\def\IEEEkeywords{\normalfont%
\@IEEEabskeysecsize\bfseries\textit{\IEEEkeywordsname}\,\bfseries\textit{---}\,%
\@IEEEgobbleleadPARNLSP}%
\def\endIEEEkeywords{\relax\vspace{0.67ex}%
\par\if@twocolumn\else\endquotation\fi%
\normalsize\normalfont}%


%%%%%
% Define \EuMWauthorrefmark to allow more flexible marking than the \IEEEauthorrefmark command
% The refmarks can now be a string of any length, of any characters.
\DeclareRobustCommand*{\EuMWauthorrefmark}[1]{\raisebox{0pt}[0pt][0pt]{\textsuperscript{\footnotesize{#1}}}}%
%
% CAUSAL PRODUCTIONS: No extra space between title and authors
\def\@IEEEauthorblockNtopspace{0ex}
% CAUSAL PRODUCTIONS: 1mm extra space between author names and affiliations
\def\@IEEEauthorblockAtopspace{1mm}
%
%%%%%%%%%%%%%%%%%%%%%%
%
\setlength{\columnsep}{6.3mm}% EuMW
\def\tablename{Table}% EuMW: was TABLE in IEEETran, but we are now using capitalized caption text not smallcaps
\def\thetable{\arabic{table}}% EuMW: Tables are numbered using arabic not roman
\def\IEEEkeywordsname{Keywords}% use Keywords instead of Index Terms
%
%%%%%%%%%%%%%%%%%%%%%%
%
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{1.5ex plus 1.5ex minus 0.5ex}%
{0.7ex plus .5ex minus 0ex}{\normalfont\normalsize\itshape}}%
%
%%%%%%%%%%%%%%%%%%%%%%
%
\setlength{\parindent}{1.5em}% make the default para indent larger to match WORD template
% define a new length that will be used for headings, so that heading title appears with same indent as paragraph
\newlength{\CPheadmatchindent}% 
\setlength{\CPheadmatchindent}{\parindent plus 0ex minus 0ex}
% define a new heading number format so that the number is in a hbox of width equal
% to the paragraph indent, so that the actual heading title will appear to be indented
% by the same amount as the paragraph below it.
\def\@seccntformat#1{\hbox to\CPheadmatchindent{\csname the#1dis\endcsname}\hskip 0.1em \relax}
%
% now we redefine the list indents so they take the new value of \parindent
\IEEEilabelindentA \parindent
\IEEEilabelindent \IEEEilabelindentA
\IEEEelabelindent \parindent
\IEEEdlabelindent \parindent
\IEEElabelindent \parindent
%%%%%%%%%%%%%%%%%%%%%%
\makeatother


